Hierarchical Uncertainty Exploration via Feedforward Posterior Trees

When solving ill-posed inverse problems, one often desires to explore the space of potential solutions rather than be presented with a single plausible reconstruction. Valuable insights into these feasible solutions and their associated probabilities are embedded in the posterior distribution. However, when confronted with data of high dimensionality (such as images), visualizing this distribution becomes a formidable challenge, necessitating the application of effective summarization techniques before user examination. In this work, we introduce a new approach for visualizing posteriors across multiple levels of granularity using tree-valued predictions. Our method predicts a tree-valued hierarchical summarization of the posterior distribution for any input measurement, in a single forward pass of a neural network. We showcase the efficacy of our approach across diverse datasets and image restoration challenges, highlighting its prowess in uncertainty quantification and visualization. Our findings reveal that our method performs comparably to a baseline that hierarchically clusters samples from a diffusion-based posterior sampler, yet achieves this with orders of magnitude greater speed.

==> 07_ack.tex <==
% add grant numbers, fruitful discussions, reviewers with helpful comments, etc.

==> texfigures/Bioimage_figure.tex <==

\begin{figure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{GT}$\\
    \includegraphics[scale=0.23]{media/main/Bioimage/img_gt.png}
\end{subfigure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{Input}$\\
\includegraphics[scale=0.23]{media/main/Bioimage/img_input.png}
\end{subfigure}

\vspace{-1.2cm}
\centering
\begin{forest}
  before typesetting nodes={
    for tree={
        font=\footnotesize,
      content/.wrap 2 pgfmath args={    {\footnotesize #2}\\\includegraphics[scale=0.23]{#1}}{content()}{title()},
    },
    where={isodd(n_children())}{calign=child, calign child/.wrap pgfmath arg={#1}{int((n_children()+1)/2)}}{},
  },
  forked edges,
  /tikz/every node/.append style={font=\footnotesize},
  for tree={
    parent anchor=children,
    child anchor=parent,
    align=center,
    l sep'= 1mm,
    s sep'= 2.5mm,
    fork sep'=0mm,
    inner sep = -2.5pt,
    edge={line width=0.5pt},
    font=\footnotesize,
  },
  [media/main/Bioimage/Level_0/img_000.png, title={ {$ \scriptstyle \text{MMSE}$}}
    [media/main/Bioimage/Level_1/img_000.png, title={ $\scriptstyle p=0.22$}
      [media/main/Bioimage/Level_2/img_000.png, title={ $\scriptstyle p=0.05$}]
      [media/main/Bioimage/Level_2/img_001.png, title={ $\scriptstyle p=0.00$}]
      [media/main/Bioimage/Level_2/img_002.png, title={ $\scriptstyle p=0.17$}]
    ]
    [media/main/Bioimage/Level_1/img_001.png, title={ $\scriptstyle p=0.19$}
      [media/main/Bioimage/Level_2/img_003.png, title={ $\scriptstyle p=0.08$}]
      [media/main/Bioimage/Level_2/img_004.png, title={ $ \scriptstyle p=0.01$}]
      [media/main/Bioimage/Level_2/img_005.png, title={ $\scriptstyle p=0.10$}]
    ]
    [media/main/Bioimage/Level_1/img_002.png, title={ $\scriptstyle p=0.59$}
      [media/main/Bioimage/Level_2/img_006.png, title={{ $\scriptstyle p=0.00$}}]
      [media/main/Bioimage/Level_2/img_007.png, title={$\scriptstyle p=0.00$}]
      [media/main/Bioimage/Level_2/img_008.png, title={ $\scriptstyle p=0.59$}]
    ]
  ]
\end{forest}
\caption{\textbf{Image to image.}}
\label{fig:bioimage2}
\end{figure}



% \begin{forest}
%   forked edges,
%   for tree={
%     align=center,
%     l sep'+= 0mm,
%     s sep'= -1mm,
%     fork sep'+=0mm,
%     edge={line width=0.5pt},
%   },
%   [MMSE\\{\includegraphics[scale=0.23]{media/main/CelebA_mouth_inpaint/Level_0/img0_000.png}},
%     % [media/main/CelebA_mouth_inpaint/Level_1/img1_000.png
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_000.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_001.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_002.png]
%     % ]
%     % [media/main/CelebA_mouth_inpaint/Level_1/img1_001.png
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_003.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_004.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_005.png]
%     % ]
%     % [media/main/CelebA_mouth_inpaint/Level_1/img1_002.png
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_006.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_007.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_008.png]
%     % ]
%   ]
% \end{forest}


==> texfigures/CelebA_colorization_figure.tex <==

\begin{figure}[t]
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{GT}$\\
    \includegraphics[scale=0.12]{media/main/CelebA_colorization/img_gt.png}
\end{subfigure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{Input}$\\
\includegraphics[scale=0.12]{media/main/CelebA_colorization/img_input.png}
\end{subfigure}


\vspace{-1.2cm}
\centering
\begin{forest}
  before typesetting nodes={
    for tree={
        font=\footnotesize,
      content/.wrap 2 pgfmath args={    {\footnotesize #2}\\\includegraphics[scale=0.12]{#1}}{content()}{title()},
    },
    where={isodd(n_children())}{calign=child, calign child/.wrap pgfmath arg={#1}{int((n_children()+1)/2)}}{},
  },
  forked edges,
  /tikz/every node/.append style={font=\footnotesize},
  for tree={
    parent anchor=children,
    child anchor=parent,
    align=center,
    l sep'= 1mm,
    s sep'= 2.5mm,
    fork sep'=0mm,
    inner sep = -2.5pt,
    edge={line width=0.5pt},
    font=\footnotesize,
  },
  [media/main/CelebA_colorization/Level_0/img_000.png, title={ {$ \scriptstyle \text{MMSE}$}}
    [media/main/CelebA_colorization/Level_1/img_000.png, title={ $\scriptstyle p=0.47$}
      [media/main/CelebA_colorization/Level_2/img_000.png, title={ $\scriptstyle p=0.19$}]
      [media/main/CelebA_colorization/Level_2/img_001.png, title={ $\scriptstyle p=0.13$}]
      [media/main/CelebA_colorization/Level_2/img_002.png, title={ $\scriptstyle p=0.14$}]
    ]
    [media/main/CelebA_colorization/Level_1/img_001.png, title={ $\scriptstyle p=0.25$}
      [media/main/CelebA_colorization/Level_2/img_003.png, title={ $\scriptstyle p=0.08$}]
      [media/main/CelebA_colorization/Level_2/img_004.png, title={ $ \scriptstyle p=0.08$}]
      [media/main/CelebA_colorization/Level_2/img_005.png, title={ $\scriptstyle p=0.09$}]
    ]
    [media/main/CelebA_colorization/Level_1/img_002.png, title={ $\scriptstyle p=0.28$}
      [media/main/CelebA_colorization/Level_2/img_006.png, title={{ $\scriptstyle p=0.19$}}]
      [media/main/CelebA_colorization/Level_2/img_007.png, title={$\scriptstyle p=0.05$}]
      [media/main/CelebA_colorization/Level_2/img_008.png, title={ $\scriptstyle p=0.04$}]
    ]
  ]
\end{forest}
\caption{\textbf{Colorization.} The predicted tree in the task of face image colorization presents various plausible colorizations varying by hat color, skin tone, and background.}
\label{fig:colorization}
\end{figure}



==> texfigures/CelebA_eye_inpaint_figure.tex <==

\begin{figure}[t]
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{GT}$\\
    \includegraphics[scale=0.12]{media/main/CelebA_eye_inpaint/img_gt.png}
\end{subfigure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{Input}$\\
\includegraphics[scale=0.12]{media/main/CelebA_eye_inpaint/img_input.png}
\end{subfigure}


\vspace{-1.2cm}
\centering
\begin{forest}
  before typesetting nodes={
    for tree={
        font=\footnotesize,
      content/.wrap 2 pgfmath args={    {\footnotesize #2}\\\includegraphics[scale=0.12]{#1}}{content()}{title()},
    },
    where={isodd(n_children())}{calign=child, calign child/.wrap pgfmath arg={#1}{int((n_children()+1)/2)}}{},
  },
  forked edges,
  /tikz/every node/.append style={font=\footnotesize},
  for tree={
    parent anchor=children,
    child anchor=parent,
    align=center,
    l sep'= 1mm,
    s sep'= 2.5mm,
    fork sep'=0mm,
    inner sep = -2.5pt,
    edge={line width=0.5pt},
    font=\footnotesize,
  },
  [media/main/CelebA_eye_inpaint/Level_0/img_000.png, title={ {$ \scriptstyle \text{MMSE}$}}
    [media/main/CelebA_eye_inpaint/Level_1/img_000.png, title={ $\scriptstyle p=0.13$}
      [media/main/CelebA_eye_inpaint/Level_2/img_000.png, title={ $\scriptstyle p=0.05$}]
      [media/main/CelebA_eye_inpaint/Level_2/img_001.png, title={ $\scriptstyle p=0.05$}]
      [media/main/CelebA_eye_inpaint/Level_2/img_002.png, title={ $\scriptstyle p=0.03$}]
    ]
    [media/main/CelebA_eye_inpaint/Level_1/img_001.png, title={ $\scriptstyle p=0.70$}
      [media/main/CelebA_eye_inpaint/Level_2/img_003.png, title={ $\scriptstyle p=0.18$}]
      [media/main/CelebA_eye_inpaint/Level_2/img_004.png, title={ $ \scriptstyle p=0.30$}]
      [media/main/CelebA_eye_inpaint/Level_2/img_005.png, title={ $\scriptstyle p=0.22$}]
    ]
    [media/main/CelebA_eye_inpaint/Level_1/img_002.png, title={ $\scriptstyle p=0.17$}
      [media/main/CelebA_eye_inpaint/Level_2/img_006.png, title={{ $\scriptstyle p=0.08$}}]
      [media/main/CelebA_eye_inpaint/Level_2/img_007.png, title={$\scriptstyle p=0.03$}]
      [media/main/CelebA_eye_inpaint/Level_2/img_008.png, title={ $\scriptstyle p=0.07$}]
    ]
  ]
\end{forest}
\caption{\textbf{Eye inpainting.} Here we illustrate our method for eye inpainting. The predicted tree explores the diverse options of eyes/eyebrows representing inherent task uncertainty.}
\label{fig:eye_inpainting}
\end{figure}



==> texfigures/CelebA_eye_inpaint_figure_v2.tex <==

% \begin{figure}[t]
% \begin{subfigure}{1cm}
%     \centering
%     $ \scriptstyle \text{GT}$\\
%     \includegraphics[scale=0.12]{media/main/CelebA_eye_inpaint/img_gt.png}
% \end{subfigure}
% \begin{subfigure}{1cm}
%     \centering
%     $ \scriptstyle \text{Input}$\\
% \includegraphics[scale=0.12]{media/main/CelebA_eye_inpaint/img_input.png}
% \end{subfigure}


% \vspace{-1.2cm}
% \centering
% \begin{forest}
%   before typesetting nodes={
%     for tree={
%         font=\footnotesize,
%       content/.wrap 2 pgfmath args={    {\footnotesize #2}\\\includegraphics[scale=0.12]{#1}}{content()}{title()},
%     },
%     where={isodd(n_children())}{calign=child, calign child/.wrap pgfmath arg={#1}{int((n_children()+1)/2)}}{},
%   },
%   forked edges,
%   /tikz/every node/.append style={font=\footnotesize},
%   for tree={
%     parent anchor=children,
%     child anchor=parent,
%     align=center,
%     l sep'= 1mm,
%     s sep'= 2.5mm,
%     fork sep'=0mm,
%     inner sep = -2.5pt,
%     edge={line width=0.5pt},
%     font=\footnotesize,
%   },
%   [media/main/CelebA_eye_inpaint/Level_0/img_000.png, title={ {$ \scriptstyle \text{MMSE}$}}
%     [media/main/CelebA_eye_inpaint/Level_1/img_000.png, title={ $\scriptstyle p=0.13$}
%       [media/main/CelebA_eye_inpaint/Level_2/img_000.png, title={ $\scriptstyle p=0.05$}]
%       [media/main/CelebA_eye_inpaint/Level_2/img_001.png, title={ $\scriptstyle p=0.05$}]
%       [media/main/CelebA_eye_inpaint/Level_2/img_002.png, title={ $\scriptstyle p=0.03$}]
%     ]
%     [media/main/CelebA_eye_inpaint/Level_1/img_001.png, title={ $\scriptstyle p=0.70$}
%       [media/main/CelebA_eye_inpaint/Level_2/img_003.png, title={ $\scriptstyle p=0.18$}]
%       [media/main/CelebA_eye_inpaint/Level_2/img_004.png, title={ $ \scriptstyle p=0.30$}]
%       [media/main/CelebA_eye_inpaint/Level_2/img_005.png, title={ $\scriptstyle p=0.22$}]
%     ]
%     [media/main/CelebA_eye_inpaint/Level_1/img_002.png, title={ $\scriptstyle p=0.17$}
%       [media/main/CelebA_eye_inpaint/Level_2/img_006.png, title={{ $\scriptstyle p=0.08$}}]
%       [media/main/CelebA_eye_inpaint/Level_2/img_007.png, title={$\scriptstyle p=0.03$}]
%       [media/main/CelebA_eye_inpaint/Level_2/img_008.png, title={ $\scriptstyle p=0.07$}]
%     ]
%   ]
% \end{forest}
% \caption{\textbf{Eye inpainting.} Here we illustrate our method for eye inpainting. The predicted tree explores the diverse options of eyes/eyebrows representing inherent task uncertainty.}
% \label{fig:eye_inpainting}
% \end{figure}

\begin{figure}[t]
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{GT}$\\
    \includegraphics[scale=0.12]{media/appendix/CelebA_eye_inpaint7/img_gt.png}
\end{subfigure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{Input}$\\
\includegraphics[scale=0.12]{media/appendix/CelebA_eye_inpaint7/img_input.png}
\end{subfigure}



\vspace{-1.2cm}
\begin{nscenter}
\begin{forest}
  before typesetting nodes={
    for tree={
        font=\footnotesize,
      content/.wrap 2 pgfmath args={    {\footnotesize #2}\\\includegraphics[scale=0.12]{#1}}{content()}{title()},
    },
    where={isodd(n_children())}{calign=child, calign child/.wrap pgfmath arg={#1}{int((n_children()+1)/2)}}{},
  },
  forked edges,
  /tikz/every node/.append style={font=\footnotesize},
  for tree={
    parent anchor=children,
    child anchor=parent,
    align=center,
    l sep'= 1mm,
    s sep'= 2.5mm,
    fork sep'=0mm,
    inner sep = -2.5pt,
    edge={line width=0.5pt},
    font=\footnotesize,
  },
  [media/appendix/CelebA_eye_inpaint7/Level_0/img_000.png, title={ {$ \scriptstyle \text{MMSE}$}}
    [media/appendix/CelebA_eye_inpaint7/Level_1/img_000.png, title={ $\scriptstyle p=0.24$}
      [media/appendix/CelebA_eye_inpaint7/Level_2/img_000.png, title={ $\scriptstyle p=0.07$}]
      [media/appendix/CelebA_eye_inpaint7/Level_2/img_001.png, title={ $\scriptstyle p=0.10$}]
      [media/appendix/CelebA_eye_inpaint7/Level_2/img_002.png, title={ $\scriptstyle p=0.07$}]
    ]
    [media/appendix/CelebA_eye_inpaint7/Level_1/img_001.png, title={ $\scriptstyle p=0.63$}
      [media/appendix/CelebA_eye_inpaint7/Level_2/img_003.png, title={ $\scriptstyle p=0.19$}]
      [media/appendix/CelebA_eye_inpaint7/Level_2/img_004.png, title={ $ \scriptstyle p=0.24$}]
      [media/appendix/CelebA_eye_inpaint7/Level_2/img_005.png, title={ $\scriptstyle p=0.21$}]
    ]
    [media/appendix/CelebA_eye_inpaint7/Level_1/img_002.png, title={ $\scriptstyle p=0.13$}
      [media/appendix/CelebA_eye_inpaint7/Level_2/img_006.png, title={{ $\scriptstyle p=0.03$}}]
      [media/appendix/CelebA_eye_inpaint7/Level_2/img_007.png, title={$\scriptstyle p=0.07$}]
      [media/appendix/CelebA_eye_inpaint7/Level_2/img_008.png, title={ $\scriptstyle p=0.03$}]
    ]
  ]
\end{forest}
\end{nscenter}
\caption{\textbf{Eyes inpainting.} Here we illustrate our method for eye inpainting. The predicted tree explores the diverse options of eyebrows/eyeglasses representing inherent task uncertainty.}
\label{fig:eye_inpainting}
\end{figure}

==> texfigures/CelebA_mouth_inpaint2_figure.tex <==

\begin{figure}[t]
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{GT}$\\
    \includegraphics[scale=0.12]{media/main/CelebA_mouth_inpaint2/img_gt.png}
\end{subfigure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{Input}$\\
\includegraphics[scale=0.12]{media/main/CelebA_mouth_inpaint2/img_input.png}
\end{subfigure}


\vspace{-1.2cm}
\centering
\begin{forest}
  before typesetting nodes={
    for tree={
        font=\footnotesize,
      content/.wrap 2 pgfmath args={    {\footnotesize #2}\\\includegraphics[scale=0.12]{#1}}{content()}{title()},
    },
    where={isodd(n_children())}{calign=child, calign child/.wrap pgfmath arg={#1}{int((n_children()+1)/2)}}{},
  },
  forked edges,
  /tikz/every node/.append style={font=\footnotesize},
  for tree={
    parent anchor=children,
    child anchor=parent,
    align=center,
    l sep'= 1mm,
    s sep'= 2.5mm,
    fork sep'=0mm,
    inner sep = -2.5pt,
    edge={line width=0.5pt},
    font=\footnotesize,
  },
  [media/main/CelebA_mouth_inpaint2/Level_0/img_000.png, title={ {$ \scriptstyle \text{MMSE}$}}
    [media/main/CelebA_mouth_inpaint2/Level_1/img_000.png, title={ $\scriptstyle p=0.06$}
      [media/main/CelebA_mouth_inpaint2/Level_2/img_000.png, title={ $\scriptstyle p=0.05$}]
      [media/main/CelebA_mouth_inpaint2/Level_2/img_001.png, title={ $\scriptstyle p=0.00$}]
      [media/main/CelebA_mouth_inpaint2/Level_2/img_002.png, title={ $\scriptstyle p=0.01$}]
    ]
    [media/main/CelebA_mouth_inpaint2/Level_1/img_001.png, title={ $\scriptstyle p=0.40$}
      [media/main/CelebA_mouth_inpaint2/Level_2/img_003.png, title={ $\scriptstyle p=0.02$}]
      [media/main/CelebA_mouth_inpaint2/Level_2/img_004.png, title={ $ \scriptstyle p=0.13$}]
      [media/main/CelebA_mouth_inpaint2/Level_2/img_005.png, title={ $\scriptstyle p=0.25$}]
    ]
    [media/main/CelebA_mouth_inpaint2/Level_1/img_002.png, title={ $\scriptstyle p=0.55$}
      [media/main/CelebA_mouth_inpaint2/Level_2/img_006.png, title={{ $\scriptstyle p=0.24$}}]
      [media/main/CelebA_mouth_inpaint2/Level_2/img_007.png, title={$\scriptstyle p=0.13$}]
      [media/main/CelebA_mouth_inpaint2/Level_2/img_008.png, title={ $\scriptstyle p=0.17$}]
    ]
  ]
\end{forest}
\caption{\textbf{Mouth inpainting.} Here we illustrate our method for mouth inpainting. The predicted tree explores the diverse options of mouth openings representing inherent task uncertainty.}
\label{fig:mouth2}
\end{figure}



==> texfigures/CelebA_mouth_inpaint3_figure.tex <==

\begin{figure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{GT}$\\
    \includegraphics[scale=0.12]{media/main/CelebA_mouth_inpaint3/img_gt.png}
\end{subfigure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{Input}$\\
\includegraphics[scale=0.12]{media/main/CelebA_mouth_inpaint3/img_input.png}
\end{subfigure}



\vspace{-1.2cm}
\centering
\begin{forest}
  before typesetting nodes={
    for tree={
        font=\footnotesize,
      content/.wrap 2 pgfmath args={    {\footnotesize #2}\\\includegraphics[scale=0.12]{#1}}{content()}{title()},
    },
    where={isodd(n_children())}{calign=child, calign child/.wrap pgfmath arg={#1}{int((n_children()+1)/2)}}{},
  },
  forked edges,
  /tikz/every node/.append style={font=\footnotesize},
  for tree={
    parent anchor=children,
    child anchor=parent,
    align=center,
    l sep'= 1mm,
    s sep'= 2.5mm,
    fork sep'=0mm,
    inner sep = -2.5pt,
    edge={line width=0.5pt},
    font=\footnotesize,
  },
  [media/main/CelebA_mouth_inpaint3/Level_0/img_000.png, title={ {$ \scriptstyle \text{MMSE}$}}
    [media/main/CelebA_mouth_inpaint3/Level_1/img_000.png, title={ $\scriptstyle p=0.10$}
      [media/main/CelebA_mouth_inpaint3/Level_2/img_000.png, title={ $\scriptstyle p=0.02$}]
      [media/main/CelebA_mouth_inpaint3/Level_2/img_001.png, title={ $\scriptstyle p=0.07$}]
      [media/main/CelebA_mouth_inpaint3/Level_2/img_002.png, title={ $\scriptstyle p=0.01$}]
    ]
    [media/main/CelebA_mouth_inpaint3/Level_1/img_001.png, title={ $\scriptstyle p=0.50$}
      [media/main/CelebA_mouth_inpaint3/Level_2/img_003.png, title={ $\scriptstyle p=0.07$}]
      [media/main/CelebA_mouth_inpaint3/Level_2/img_004.png, title={ $ \scriptstyle p=0.15$}]
      [media/main/CelebA_mouth_inpaint3/Level_2/img_005.png, title={ $\scriptstyle p=0.29$}]
    ]
    [media/main/CelebA_mouth_inpaint3/Level_1/img_002.png, title={ $\scriptstyle p=0.40$}
      [media/main/CelebA_mouth_inpaint3/Level_2/img_006.png, title={{ $\scriptstyle p=0.14$}}]
      [media/main/CelebA_mouth_inpaint3/Level_2/img_007.png, title={$\scriptstyle p=0.17$}]
      [media/main/CelebA_mouth_inpaint3/Level_2/img_008.png, title={ $\scriptstyle p=0.10$}]
    ]
  ]
\end{forest}
\caption{\textbf{Mouth inpainting.}}
\end{figure}



% \begin{forest}
%   forked edges,
%   for tree={
%     align=center,
%     l sep'+= 0mm,
%     s sep'= -1mm,
%     fork sep'+=0mm,
%     edge={line width=0.5pt},
%   },
%   [MMSE\\{\includegraphics[scale=0.12]{media/main/CelebA_mouth_inpaint/Level_0/img0_000.png}},
%     % [media/main/CelebA_mouth_inpaint/Level_1/img1_000.png
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_000.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_001.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_002.png]
%     % ]
%     % [media/main/CelebA_mouth_inpaint/Level_1/img1_001.png
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_003.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_004.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_005.png]
%     % ]
%     % [media/main/CelebA_mouth_inpaint/Level_1/img1_002.png
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_006.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_007.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_008.png]
%     % ]
%   ]
% \end{forest}


==> texfigures/Shoes2_figure.tex <==

\begin{figure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{GT}$\\
    \includegraphics[scale=0.12]{media/main/Shoes2/img_gt.png}
\end{subfigure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{Input}$\\
\includegraphics[scale=0.12]{media/main/Shoes2/img_input.png}
\end{subfigure}



\vspace{-1.2cm}
\centering
\begin{forest}
  before typesetting nodes={
    for tree={
        font=\footnotesize,
      content/.wrap 2 pgfmath args={    {\footnotesize #2}\\\includegraphics[scale=0.12]{#1}}{content()}{title()},
    },
    where={isodd(n_children())}{calign=child, calign child/.wrap pgfmath arg={#1}{int((n_children()+1)/2)}}{},
  },
  forked edges,
  /tikz/every node/.append style={font=\footnotesize},
  for tree={
    parent anchor=children,
    child anchor=parent,
    align=center,
    l sep'= 1mm,
    s sep'= 2.5mm,
    fork sep'=0mm,
    inner sep = -2.5pt,
    edge={line width=0.5pt},
    font=\footnotesize,
  },
  [media/main/Shoes2/Level_0/img_000.png, title={ {$ \scriptstyle \text{MMSE}$}}
    [media/main/Shoes2/Level_1/img_000.png, title={ $\scriptstyle p=0.04$}
      [media/main/Shoes2/Level_2/img_000.png, title={ $\scriptstyle p=0.04$}]
      [media/main/Shoes2/Level_2/img_001.png, title={ $\scriptstyle p=0.00$}]
      [media/main/Shoes2/Level_2/img_002.png, title={ $\scriptstyle p=0.00$}]
    ]
    [media/main/Shoes2/Level_1/img_001.png, title={ $\scriptstyle p=0.95$}
      [media/main/Shoes2/Level_2/img_003.png, title={ $\scriptstyle p=0.95$}]
      [media/main/Shoes2/Level_2/img_004.png, title={ $ \scriptstyle p=0.00$}]
      [media/main/Shoes2/Level_2/img_005.png, title={ $\scriptstyle p=0.00$}]
    ]
    [media/main/Shoes2/Level_1/img_002.png, title={ $\scriptstyle p=0.01$}
      [media/main/Shoes2/Level_2/img_006.png, title={{ $\scriptstyle p=0.01$}}]
      [media/main/Shoes2/Level_2/img_007.png, title={$\scriptstyle p=0.00$}]
      [media/main/Shoes2/Level_2/img_008.png, title={ $\scriptstyle p=0.00$}]
    ]
  ]
\end{forest}
\caption{\textbf{Image to image.}}
\end{figure}



% \begin{forest}
%   forked edges,
%   for tree={
%     align=center,
%     l sep'+= 0mm,
%     s sep'= -1mm,
%     fork sep'+=0mm,
%     edge={line width=0.5pt},
%   },
%   [MMSE\\{\includegraphics[scale=0.12]{media/main/CelebA_mouth_inpaint/Level_0/img0_000.png}},
%     % [media/main/CelebA_mouth_inpaint/Level_1/img1_000.png
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_000.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_001.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_002.png]
%     % ]
%     % [media/main/CelebA_mouth_inpaint/Level_1/img1_001.png
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_003.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_004.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_005.png]
%     % ]
%     % [media/main/CelebA_mouth_inpaint/Level_1/img1_002.png
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_006.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_007.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_008.png]
%     % ]
%   ]
% \end{forest}


==> texfigures/Shoes3_figure.tex <==

\begin{figure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{GT}$\\
    \includegraphics[scale=0.12]{media/main/Shoes3/img_gt.png}
\end{subfigure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{Input}$\\
\includegraphics[scale=0.12]{media/main/Shoes3/img_input.png}
\end{subfigure}



\vspace{-1.2cm}
\centering
\begin{forest}
  before typesetting nodes={
    for tree={
        font=\footnotesize,
      content/.wrap 2 pgfmath args={    {\footnotesize #2}\\\includegraphics[scale=0.12]{#1}}{content()}{title()},
    },
    where={isodd(n_children())}{calign=child, calign child/.wrap pgfmath arg={#1}{int((n_children()+1)/2)}}{},
  },
  forked edges,
  /tikz/every node/.append style={font=\footnotesize},
  for tree={
    parent anchor=children,
    child anchor=parent,
    align=center,
    l sep'= 1mm,
    s sep'= 2.5mm,
    fork sep'=0mm,
    inner sep = -2.5pt,
    edge={line width=0.5pt},
    font=\footnotesize,
  },
  [media/main/Shoes3/Level_0/img_000.png, title={ {$ \scriptstyle \text{MMSE}$}}
    [media/main/Shoes3/Level_1/img_000.png, title={ $\scriptstyle p=0.04$}
      [media/main/Shoes3/Level_2/img_000.png, title={ $\scriptstyle p=0.00$}]
      [media/main/Shoes3/Level_2/img_001.png, title={ $\scriptstyle p=0.00$}]
      [media/main/Shoes3/Level_2/img_002.png, title={ $\scriptstyle p=0.04$}]
    ]
    [media/main/Shoes3/Level_1/img_001.png, title={ $\scriptstyle p=0.54$}
      [media/main/Shoes3/Level_2/img_003.png, title={ $\scriptstyle p=0.54$}]
      [media/main/Shoes3/Level_2/img_004.png, title={ $ \scriptstyle p=0.00$}]
      [media/main/Shoes3/Level_2/img_005.png, title={ $\scriptstyle p=0.00$}]
    ]
    [media/main/Shoes3/Level_1/img_002.png, title={ $\scriptstyle p=0.41$}
      [media/main/Shoes3/Level_2/img_006.png, title={{ $\scriptstyle p=0.37$}}]
      [media/main/Shoes3/Level_2/img_007.png, title={$\scriptstyle p=0.02$}]
      [media/main/Shoes3/Level_2/img_008.png, title={ $\scriptstyle p=0.03$}]
    ]
  ]
\end{forest}
\caption{\textbf{Image to image.}}
\end{figure}



% \begin{forest}
%   forked edges,
%   for tree={
%     align=center,
%     l sep'+= 0mm,
%     s sep'= -1mm,
%     fork sep'+=0mm,
%     edge={line width=0.5pt},
%   },
%   [MMSE\\{\includegraphics[scale=0.12]{media/main/CelebA_mouth_inpaint/Level_0/img0_000.png}},
%     % [media/main/CelebA_mouth_inpaint/Level_1/img1_000.png
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_000.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_001.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_002.png]
%     % ]
%     % [media/main/CelebA_mouth_inpaint/Level_1/img1_001.png
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_003.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_004.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_005.png]
%     % ]
%     % [media/main/CelebA_mouth_inpaint/Level_1/img1_002.png
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_006.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_007.png]
%     %   [media/main/CelebA_mouth_inpaint/Level_2/img2_008.png]
%     % ]
%   ]
% \end{forest}


==> texfigures/Shoes_figure.tex <==

\begin{figure}[t]
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{GT}$\\
    \includegraphics[scale=0.12]{media/main/Shoes/img_gt.png}
\end{subfigure}
\begin{subfigure}{1cm}
    \centering
    $ \scriptstyle \text{Input}$\\
\includegraphics[scale=0.12]{media/main/Shoes/img_input.png}
\end{subfigure}


\vspace{-1.2cm}
\centering
\begin{forest}
  before typesetting nodes={
    for tree={
        font=\footnotesize,
      content/.wrap 2 pgfmath args={    {\footnotesize #2}\\\includegraphics[scale=0.12]{#1}}{content()}{title()},
    },
    where={isodd(n_children())}{calign=child, calign child/.wrap pgfmath arg={#1}{int((n_children()+1)/2)}}{},
  },
  forked edges,
  /tikz/every node/.append style={font=\footnotesize},
  for tree={
    parent anchor=children,
    child anchor=parent,
    align=center,
    l sep'= 1mm,
    s sep'= 2.5mm,
    fork sep'=0mm,
    inner sep = -2.5pt,
    edge={line width=0.5pt},
    font=\footnotesize,
  },
  [media/main/Shoes/Level_0/img_000.png, title={ {$ \scriptstyle \text{MMSE}$}}
    [media/main/Shoes/Level_1/img_000.png, title={ $\scriptstyle p=0.31$}
      [media/main/Shoes/Level_2/img_000.png, title={ $\scriptstyle p=0.16$}]
      [media/main/Shoes/Level_2/img_001.png, title={ $\scriptstyle p=0.10$}]
      [media/main/Shoes/Level_2/img_002.png, title={ $\scriptstyle p=0.05$}]
    ]
    [media/main/Shoes/Level_1/img_001.png, title={ $\scriptstyle p=0.61$}
      [media/main/Shoes/Level_2/img_003.png, title={ $\scriptstyle p=0.01$}]
      [media/main/Shoes/Level_2/img_004.png, title={ $ \scriptstyle p=0.49$}]
      [media/main/Shoes/Level_2/img_005.png, title={ $\scriptstyle p=0.11$}]
    ]
    [media/main/Shoes/Level_1/img_002.png, title={ $\scriptstyle p=0.09$}
      [media/main/Shoes/Level_2/img_006.png, title={{ $\scriptstyle p=0.00$}}]
      [media/main/Shoes/Level_2/img_007.png, title={$\scriptstyle p=0.03$}]
      [media/main/Shoes/Level_2/img_008.png, title={ $\scriptstyle p=0.05$}]
    ]
  ]
\end{forest}
\caption{\textbf{Edges$\rightarrow$Shoes.} Here we demonstrate posterior trees on translating edge images to shoes. The predicted tree refines the mean estimate by color, grouping similar colors, while still depicting unlikely ones (\eg the blue boot).}
\label{fig:shoes}
\end{figure}



